Optimizing Joint Probabilistic Caching and Communication for Clustered D2D Networks

Caching at mobile devices and leveraging device-to-device (D2D) communication are two promising approaches to support massive content delivery over wireless networks. The analysis of such D2D caching networks based on a physical interference model is usually carried out by assuming that devices are uniformly distributed. However, this approach does not fully consider and characterize the fact that devices are usually grouped into clusters. Motivated by this fact, this paper presents a comprehensive performance analysis and joint communication and caching optimization for a clustered D2D network. Devices are distributed according to a Thomas cluster process (TCP) and are assumed to have a surplus memory which is exploited to proactively cache files from a known library, following a random probabilistic caching scheme. Devices can retrieve the requested files from their caches, from neighbouring devices in their proximity (cluster), or from the base station as a last resort. Three key performance metrics are optimized in this paper, namely, the offloading gain, energy consumption, and latency.

==> IEEE TWC 2019/acronyms.tex <==

\acro{D2D}{device-to-device}
\acro{SIR}{signal to interference ratio}
\acro{SINR}{signal to interference plus noise ratio}
\acro{PCP}{Poisson cluster process}
\acro{CoMP}{coordinated multi-point}
\acro{BS}{base station} 
\acro{MD-CoMP}{macrodiversity CoMP transmission}
\acro{MAC}{medium-access-control}
\acro{JT-CoMP}{joint transmission CoMP}
\acro{CoMP-JT}{coordinated multipoint joint transmission}
\acro{SBS}{small base station}
\acro{MDSD}{multiple devices to the single device}
\acro{MDS}{maximum distance seperable}
\acro{SCN}{small cell network}
\acro{PPP}{Poisson point process}
\acro{TCP}{Thomas cluster process}
\acro{CSI}{channel state information}
\acro{PDF}{probability distribution function}
\acro{PMF}{probability mass function}
\acro{RV}{random variable}
\acro{i.i.d.}{independently and identically distributed}
\acro{MBMS}{multimedia broadcasting multicasting service}
\acro{EE}{energy efficiency}
\acro{HCP}{hard-core placement}
\acro{CCDF}{complementary cumulative distribution function}
\acro{PC}{probabilistic caching}
\acro{RC}{random uniform caching}
\acro{CPF}{caching popular files} 
\acro{BCD}{block coordinate descent}
\acro{CTMC}{continuous-time Markov chain}
\acro{PGFL}{point generating functional}
\acro{KKT}{Karush-Kuhn-Tucker}
%\acro{}{}
%\acro{}{}
%\acro{}{}
%\acro{}{}
%\acro{}{}
%\acro{}{}
%\acro{}{}
%\acro{}{}
%\acro{}{}


==> IEEE TWC 2019/newcommands.tex <==


\newcommand{\sinr}{\mathrm{SINR}}
\newcommand{\sir}{\mathrm{SIR}}
\newcommand{\pc}{\mathrm{P_c}}
\newcommand{\pcd}{\mathrm{P_{c_d}}}
\newcommand{\pcb}{\mathrm{P_{c_b}}}
\newcommand{\Pb}{\mathbb{P}}
\newcommand{\Eb}{\mathbb{E}}
\newcommand{\Rb}{\mathbb{R}}
\newcommand{\Rs}{\mathbb{R}^2}
\newcommand{\Rp}{\mathbb{R}^+}
\newcommand{\Lc}{\mathcal{L}} 
\newcommand{\e}{\mathcal{E}} 
\newcommand{\eav}{\mathcal{E_{av}}} 

\newcommand{\besselI}[1]{\mbox{I$_0$}(#1)}

